Blind Inversion using Latent Diffusion Priors

Diffusion models have emerged as powerful tools for solving inverse problems due to their exceptional ability to model complex prior distributions. However, existing methods predominantly assume known forward operators (i.e., non-blind), limiting their applicability in practical settings where acquiring such operators is costly. Additionally, many current approaches rely on pixel-space diffusion models, leaving the potential of more powerful latent diffusion models (LDMs) underexplored. In this paper, we introduce LatentDEM, an innovative technique that addresses more challenging blind inverse problems using latent diffusion priors. At the core of our method is solving blind inverse problems within an iterative Expectation-Maximization (EM) framework: (1) the E-step recovers clean images from corrupted observations using LDM priors and a known forward model, and (2) the M-step estimates the forward operator based on the recovered images. Additionally, we propose two novel optimization techniques tailored for LDM priors and EM frameworks, yielding more accurate and efficient blind inversion results. As a general framework, LatentDEM supports both linear and non-linear inverse problems. Beyond common 2D image restoration tasks, it enables new capabilities in non-linear 3D inverse rendering problems. We validate LatentDEM's performance on representative 2D blind deblurring and 3D sparse-view reconstruction tasks, demonstrating its superior efficacy over prior arts.

==> Styles/chapter/2-introduction.tex <==
\section{Introduction}
Inverse problems aim to recover underlying signals $\boldsymbol{x}$, from partial and corrupted observations $\boldsymbol{y}$ generated by a forward operator $\mathcal{A}_{\phi}(\cdot)$. 
Such problems are prevalent in computational imaging, including denoising, deblurring, inpainting, and 3D reconstruction. 
Typically, inverse problem solvers assume knowing the forward model and its physical parameters, $\phi$ (i.e., \textit{non-blind}). 
However, acquiring accurate forward models is often challenging or impractical in real-world settings, necessitating a more complex task of solving \textit{blind} inverse problems, where both the hidden signals $\boldsymbol{x}$ and the forward model parameters $\phi$ must be jointly estimated.

Diffusion models (DMs) have emerged as powerful tools for solving inverse problems. Unlike traditional supervised learning approaches that train an end-to-end neural network to map observations directly to hidden images ($\boldsymbol{y} \to \boldsymbol{x}$), DMs approximate the prior distribution of underlying signals, $p(x)$, by learning the distribution's score function, $\nabla_x \log p(x)$, through a neural network. This approach allows data driven priors to be integrated into Bayesian inverse problem solvers as a replacement for conventional handcrafted priors (e.g., total variation, sparsity), facilitating reconstruction of hidden images in an unsupervised learning manner. Recently, latent diffusion models (LDMs) have set a new standard by creating foundational generative models across domains. LDMs project signals into a lower-dimensional latent space, $z=\mathcal{E}\left(x\right)$, perform diffusion there using latent score function, $\nabla_z \log p(z)$, and then decode the latent state back to the pixel space, $x=\mathcal{D}\left(z\right)$. This strategy mitigates the curse of dimensionality typical in pixel-space DMs and reveals superior capability, flexibility, and efficiency in modeling complex, high-dimensional distributions, such as those of videos, audios, and 3D objects.

Although both DM-based and LDM-based solvers have demonstrated impressive posterior sampling performance in diverse computational imaging inverse problems, existing methods predominantly focus on non-blind settings. Blind inversion poses non-convex optimization challenges, often leading to instabilities when jointly solving for model parameters and underlying images. While recent advances have explored the feasibility of solving blind inverse problems using pixel-based DMs, these methods suffer from computational inefficiencies and limited capability in modeling complex image priors, rendering them unsuitable for high-dimensional blind inversion tasks like 3D imaging.

In this paper, we introduce LatentDEM, a general framework to address blind inverse problems using pre-trained LDMs. The core concept of LatentDEM involves a variational expectation-maximization (EM) framework that alternates between reconstructing underlying images through latent diffusion posterior sampling (E-step) and estimating forward model parameters using the reconstructed images (M-step). We also implement an annealed optimization scheme to enhance the stability of LatentDEM training, particularly in early stages when the model parameters may significantly deviate from their true values. By decoupling image reconstruction and model parameter updates into separate steps, LatentDEM significantly reduces the computational burden associated with LDM’s encoder-decoder processes. This allows us to leverage the capabilities of pre-trained foundational diffusion models, such Stable Diffusion, to solve a wide range of blind inverse problems effectively. We validate our method on two challenging blind inversion tasks, blind motion deblurring and pose-free sparse-view 3D reconstruction, and achieve new state-of-the-art performance in both imaging quality and efficiency.


% Inverse problems aim to recover underlying signals from partial observations generated by the forward operators.
% These problems widely exist in computational imaging, such as image deblurring, inpainting and denoising.
% Most physical-based algorithms assume the knowledge of forward operators and the corresponding parameters, that is, \textit{non-blind} inverse problem.
% Nevertheless, in real-world scenarios, forward operators with corresponding parameters are hard to acquire, resulting in \textit{blind} inverse problems where the operators are unknown.
% The latter problem is considered harder to solve, as the joint optimization of images and forward operators is not stable.

% Recently, Diffusion models (DMs) have emerged as powerful solvers for inverse problems.
% In DMs, original data are gradually corrupted into pure Gaussian noise in the diffusion process. 
% Reversely, the noise is eliminated with deep neural networks in the generative process to learn the underlying score function of data distribution.
% Advanced researches in the field of inverse problems broadly adopt pre-trained DMs as versatile priors, achieving state-of-the-art performance in non-blind inverse imaging.
% Commonly, diffusion-based inverse problem solvers adapt the standard generative process into the posterior sampling process by applying the Bayesian rule. 
% They perform posterior sampling by calculating the prior term with pre-trained DMs and the likelihood term for data consistency.
% The likelihood term usually requires the knowledge of the forward operators, along with the corresponding parameters (i.e. blur kernel, mask matrix, noisy level map).
% Considering the forward operators are expensive or even impossible to acquire, we argue that traditional diffusion posterior sampling methods are not consistent with real-world cases.
% Only few researchers have focused on solving blind inverse problems based on DMs~\cite{chung2022parallel, laroche2024fast}.


\begin{figure*}[tbp]
\centering
\includegraphics[width=13.cm]{Styles/figure/blindinverse-teaser.pdf}
\centering
\caption{\textbf{Representative results of the proposed method.}  We conduct two blind inverse problems,
motion deblurring and multi-view consistent 3D modeling without poses, on blurry observations and 2D views, respectively. Notably, our method estimates the kernels and poses accurately.}
\label{fig:exp-aba-annealing}
\end{figure*}

% BlindDPS~\cite{chung2022parallel} designs a parallel optimization paradigm by adding a forward operator diffusion besides the image diffusion.
% Fast diffusion EM~\cite{laroche2024fast} proposes to replace the forward operator diffusion with an explicit deconvolution scheme plus a plug-and-play denoiser, therefore accelerating the inverse process.

% However, previous works are limited to the pixel-space DMs in the field of blind inverse problems for stability. 
% They need domain-specific diffusion priors for each specific domain image restoration, leaving the usage of foundation diffusion priors based on latent space unexplored.
% Moreover, pixel-space DMs often suffer from low computational efficiency due to their high-dimensional training space, thus failing in complex imaging such as blind inversion and 3D modeling. 
% Latent diffusion models (LDMs) increase computational efficiency significantly by embedding data into a lower-dimensional space, making various imaging and 3D modeling feasible and efficient.
% In this paper, we propose LatentDEM, the first latent diffusion-based blind inverse problem solver.
% LatentDEM utilizes a variational expectation-maximum framework to jointly learn underlying signals and forward operators, with latent diffusion models and forward operator estimators respectively.
% We propose an {annealed} optimization scheme to address the instability of LDMs for blind inverse problems. 
% We further decouple the joint optimization to reduce the computation from the encoder-decoder process.
% It brings two fundamental advantages: cross-domain diffusion priors and fewer computation overhead, which are crucial for solving blind inverse problems.
% Concretely, our method has two key components:
% (1) E-step: endow the generative process with a foundation latent diffusion model,
% (2) M-step: estimate the forward operator with a carefully designed estimator.
% Theoretical analysis of the blind posterior sampling and convergence guarantee is provided.

% In fact, LatentDEM can be seen as a universal inverse problem solver: no need for domain-specific priors nor the knowledge of forward operators, thus can be applied to solve various real-world 2D and 3D inverse problems effectively and efficiently.
% We demonstrate our method on two blind inverse tasks, blind motion deblurring and sparse-view consistent 3D modeling without poses. 
% From our experimental results, LatentDEM outperforms baselines significantly, achieving state-of-the-art performance in the quality of imaging, and increasing the computation efficiency.

% In summary, the contributions of this paper are:
% \begin{itemize}[leftmargin=*,itemindent=0mm, noitemsep]
%     \item We propose the first universal inverse problem solver LatentDEM, without a need for domain-specific priors nor the knowledge of forward operators.
%     \item Two improved techniques are designed for solving blind inverse problems with latent diffusion models (LDMs) effectively and efficiently.
%     \item Theoretical analysis of the latent diffusion models for blind inverse problems and the convergence guarantee is provided.
%     \item Our method achieves new state-of-the-art performance on 2D and 3D blind inverse problems in the quality of imaging, and significantly reduces the computation overhead.
% \end{itemize}

==> Styles/chapter/3-background.tex <==
\section{Background}

\subsection{Blind Inverse Problems}
The goal of general inverse problems is to recover signals $\boldsymbol{x}\in \mathbb{R}^D$ from partial observations $\boldsymbol{y}\in \mathbb{R}^M $:
\begin{equation}
    \boldsymbol{y}=\mathcal{A}_{\phi}\left(\boldsymbol{x}\right)+\boldsymbol{n},
\label{equ: inverse}
\end{equation}
where $\phi$ is the parameters of forward operator $\mathcal{A}$, $\boldsymbol{n}$ is some noise. 
Considering $\boldsymbol{y}$ usually misses information about underlying $\boldsymbol{x}$, solving inverse problems is ill-posed. 
Depending on whether $\phi$ is known, inverse problems can be divided into two categories: \textit{non-blind} inverse problems and \textit{blind} inverse problems.
The latter has to jointly estimate $\boldsymbol{x}$ and $\phi$, thus are considered to be consistent with real-world scenarios but much harder.
In this paper, we focus on solving blind inverse problems with state-of-the-art latent diffusion models.


% Definition of general inverse problems.
% there is already a lot of work on leveraging the diffusion model to solve various inverse problem tasks,like inpainting, super-resolution and motion deblur(Song et al., 2021b\cite{song2021scorebased}; Chung & Ye, 2022\cite{chung2022parallel}; Chung et al.,2022b; Rout et al.,2023\cite{NEURIPS2023_9c70cfa2}), but these work all assumes that we already have complete knowledge about the forward operator $\mathcal{A}$, which can not be known in advance in reality. To make full use of the diffusion model, we should consider the case that the forward operator is unknown\cite{chung2022parallel}. Among them, we focus on the case where the forward operator is
% parameterized with $\phi$, which is also needed to estimate during the diffusion process. Specifically, consider the following forward model:


\subsection{Diffusion models}
We first briefly review the basic fundamentals of diffusion models (DMs), namely the score-based models~\cite{ho2020denoising, song2021scorebased, sohl2015deep}. 
They are powerful generative models by learning the score function $\nabla_{\boldsymbol{x}} \log p(\boldsymbol{x})$ of data distribution.
Specifically, DMs start by progressively injecting Gaussian noise into data, which can be described as a forward-time stochastic differential equation (SDE)~\cite{song2021scorebased}:
\begin{equation}
     \mathrm{d} \boldsymbol{x}=-\frac{\beta(t)}{2}\boldsymbol{x} \mathrm{d} t+\sqrt{\beta(t)} \mathrm{d} \boldsymbol{w},
\label{equ:diffusion}
\end{equation}
where $\beta(t)\in(0,1)$ is the noise schedule and $\boldsymbol{w}$ is the standard Wiener process.
This equation is also called variance-preserving SDE (VP-SDE), which equals DDPM~\cite{ho2020denoising}.
A proper noise schedule perturbs data distribution $p(\boldsymbol{x})$ into standard Gaussian distribution $\mathcal{N}(\boldsymbol{0}, \boldsymbol{I})$.
Then, the generative reverse SDE is formulated as:
\begin{equation}
    \mathrm{d} \boldsymbol{x}=\left[-\frac{\beta({t})}{2} \boldsymbol{x}-\beta({t}) \nabla_{\boldsymbol{x}_{t}} \log p\left(\boldsymbol{x}_{t}\right)\right] \mathrm{d} t+\sqrt{\beta({t})} \mathrm{d} \overline{\boldsymbol{w}},
\label{equ:reversesde}
\end{equation}
where the score function $\nabla_{\boldsymbol{x}_{t}} \log p\left(\boldsymbol{x}_{t}\right)$ is approximated by parameterized deep neural networks $\boldsymbol{s}_\theta$, and $\overline{\boldsymbol{w}}$ is the standard Wiener process running backward in time. 
Solving this equation equals generating data from standard Gaussian noise.
One can train $\boldsymbol{s}_\theta$ via denoising score matching~\cite{vincent2011connection}:
\begin{equation}
    \hat{\theta}=\underset{\theta}{\arg \min } \mathbb{E}\left[\left\|\boldsymbol{s}_{\theta}\left(\boldsymbol{x}_{t}, t\right)-\nabla_{\boldsymbol{x}_{t}} \log p\left(\boldsymbol{x}_{t}| \boldsymbol{x}_{0}\right)\right\|_{2}^{2}\right]
\end{equation}
where $t$ is sampled from $[0,T]$ uniformly and the expectation is taken over all the time step $t$ that we choose. 
Once the score-estimating neural network is learned, $\boldsymbol{s}_\theta$ can be used to solve Eq.~\ref{equ:reversesde} via ancestral sampling~\cite{ho2020denoising}, drawing samples from $p(\boldsymbol{x})$.

\paragraph{Latent diffusion models.}
A significant drawback of pixel-based DMs is that they require substantial computational resources and a large volume of training data.
To reduce the computation overhead, a generalized family of Latent Diffusion Models (LDMs) is proposed~\cite{rombach2022high, blattmann2023align}.
LDMs embed data into a compressed latent space for efficiency and flexibility:
\begin{equation}
    \boldsymbol{z}=\mathcal{E}(\boldsymbol{x}), \boldsymbol{x}=\mathcal{D}(\boldsymbol{z}),
\end{equation}
where $\mathcal{E}: \mathbb{R}^D\to\mathbb{R}^N$ is an encoder, $\mathcal{D}: \mathbb{R}^N\to\mathbb{R}^D$ is a corresponding decoder, and $N\ll D$.
LDMs power state-of-the-art foundation models such as Stable Diffusion~\cite{rombach2022high}, which can serve as a powerful cross-domain prior.
% However, LDMs are notorious for their instability due to the vulnerability of latent space.
The versatility of LDMs makes them promising solvers for inverse problems.
Notably, such an efficient paradigm is a double-edged sword, as LDMs are notorious for their instability due to the vulnerability of latent space~\cite{rout2024solving, chung2023prompt}.


\subsection{Diffusion models for inverse problems}
A common approach to solving non-blind inverse problems in Eq.~\ref{equ: inverse} is to adopt the Bayesian framework: $p(\boldsymbol{x}|\boldsymbol{y})\propto p(\boldsymbol{x})p(\boldsymbol{y}|\boldsymbol{x})$, where one can acquire the posterior $p(\boldsymbol{x}|\boldsymbol{y})$ with prior $p(\boldsymbol{x})$ and likelihood $p(\boldsymbol{y}|\boldsymbol{x})$. 
We can leverage pre-trained DMs as generative priors and modify the score function as:
\begin{equation}
    \nabla_{\boldsymbol{x}_{t}} \log p_{t}\left(\boldsymbol{x}_t|\boldsymbol{y}\right)=
    \nabla_{\boldsymbol{x}_{t}} \log p_{t}\left(\boldsymbol{x}_{t}\right)
    +\nabla_{\boldsymbol{x}_{t}} \log p_{t}\left(\boldsymbol{y}|\boldsymbol{x}_{t}\right),
\end{equation}
where $\nabla_{\boldsymbol{x}_{t}} \log p_{t}\left(\boldsymbol{x}_{t}\right)$ can be approximated by a pre-trained DM $\boldsymbol{s}_\theta$ and $\nabla_{\boldsymbol{x}_{t}} \log p_{t}\left(\boldsymbol{y}|\boldsymbol{x}_{t}\right)$ is a time-dependent likelihood defined by an intractable integral over all $\boldsymbol{x}$. 
Previous methods resolve this problem by either abandoning the direct use of the likelihood~\cite{adam2022posterior, chung2022come, chung2022score, wang2022zero} or approximating the likelihood~\cite{chung2022diffusion, song2021solving, feng2023efficient}. 
Recently, \cite{rout2024solving, song2023solving} propose to solve non-blind inverse problems with LDMs.
However, diffusion-based solvers for blind inverse problems are all limited to pixel-based DMs~\cite{chung2022parallel, laroche2024fast}, as the instability of LDMs makes the joint optimization even harder.
In this paper, we investigate how to cooperate with powerful LDMs for solving blind inverse problems. 


==> Styles/chapter/4-Method-v1.tex <==


\vspace*{-0.1cm}
\section{Method}
We describe how to solve \emph{blind} inverse problems using latent diffusion priors. Our method is formulated within a variational Expectation-Maximization (EM) framework, where the signals and forward operators are iteratively optimized through EM iterations. In the E-step (Sec.\ref{sec:E-step}), we leverage latent diffusion priors to draw signal posterior samples. In the M-step (Sec.\ref{sec:M-step}), we estimate forward operators in a maximum-a-posteriori (MAP) manner. To improve the stability and efficiency of blind inversion, we propose a scheduling method for arranging the execution of the E-steps and M-steps in Sec.\ref{sec:EM framework}. In Sec.\ref{sec:app}, we show how our framework can be applied to solve representative problems such as 2D blind deblurring and 3D pose-free sparse-view reconstruction.

% We now describe how to solve \emph{blind} inverse problem with latent diffusion priors.
% Our method is formulated in a variational expectation-maximum (EM) framework, where the signals and the forward operators are iteratively optimized through EM iterations.
% In the E-step(Sec.~\ref{sec:E-step}), we leverage the versatile latent diffusion priors to draw signal posterior samples; while in the M-step(Sec.~\ref{sec:M-step}), we estimate forward operators via a maximum-a-posterior (MAP) manner.
% To improve the stability and efficiency of for the blind inversion, in Sec.~\ref{sec:EM framework}, we also propose a scheduling method for aranging the execution of the E-steps and M-steps. In Sec.~\ref{sec:app}, we show our framework can be applied to solve the representative 2D blind debluring and 3D pose-free sparse-view reconstruction problems.
%
% Being a double-edged sword, latent diffusion priors could yield better performance but are also extremely vulnerable. We then propose a optimization techniques to xxxx. %We show simply bridging LDM priors in EM framework produces results with significant artificats and carefully designs gradients optimization scheme and EM scheduling to enhance training stability and efficiency, and provide the convergence guarantee in Sec.~\ref{sec:EM framework}. \wz{refine}
% To that end, we study a variational expectation-maximum framework for joint optimization of signals and forward operators, as shown in Figure~\ref{fig:overview}.
% Iteratively, we first leverage the versatility of large-scale latent diffusion models to draw samples in E-step (Section~\ref{sec:E-step}), then we estimate forward operators via maximum a posterior in M-step (Section~\ref{sec:M-step}). We further propose two techniques for stability and acceleration, and provide the convergence guarantee (Section~\ref{sec:EM framework}).


% $\probDistribution{\signal | \observation, \pretrainSdModel, \forwardFunc_\forwardParam}$
% , where $\pretrainSdModel$ is the score function of a pretrained diffusion model. 
\subsection{E-step: Posterior Sampling via Latent Diffusion}
\label{sec:E-step}
The goal of {\name}'s E-step is to solve for the posterior distribution $p_{\phi}(\signal \mid \observation)$ by leveraging the reverse time SDE in Eq.~\ref{equ:diffusion}. 
To utilize the latent priors, inspired by latentDPS~\cite{rout2024solving}, we conduct posterior sampling in the  latent space by defining a conditional latent diffusion process: % where  the  score function $\scoreFunc{\signal_\noisetime}{\signal_\noisetime | \observation}$ is transformed as $\scoreFunc{\latent_\noisetime}{\latent_\noisetime | \observation}$:
%
	\begin{align}
		\scoreFunc{\latent_\noisetime}{\latent_\noisetime \mid \observation}
		&=
		\scoreFunc{\latent_\noisetime}{\latent_\noisetime}
		+ 	\scoreFunc{\latent_\noisetime}{ \observation \mid \latent_t} 
		\\
		% \scoreFunc{\latent_\noisetime}{ \observation \mid \latent_t}
        &\approx \pretrainSdModel{(\latent_\noisetime, \noisetime)} + \nabla_{\latent_\noisetime} \log p_{\phi} ({ \observation \mid \pretraiedDecodeFunc{\mathbb{E}[{\latent}_{0}| \latent_{t}]} })\\
        &= \pretrainSdModel{(\latent_\noisetime, \noisetime)} - \frac{1}{2\sigma^{2}} \nabla_{\mathbf{x}_{t}}\left\|\mathbf{y}-\mathcal{A}_\phi\left( \pretraiedDecodeFunc{\mathbb{E}[{\latent}_{0}| \latent_{t}]}\right)\right\|_{2}^{2}
        % \nabla_{\latent_\noisetime} \log p_{\phi} ({ \observation \mid \pretraiedDecodeFunc{\mathbb{E}[{\latent}_{0}| \latent_{t}]} }),
   %      &\approx
			% \nabla_{\latent_\noisetime} \log p ({ \observation \mid \pretraiedDecodeFunc{\mathbb{E}[{\latent}_{0}| \latent_{t}]} }).
	\label{equ: blindinverse1}
	\end{align}
%
where $\pretrainSdModel{(\latent_\noisetime, \noisetime)}$ is the pre-trained LDM that approximates the latent score function $\scoreFunc{\latent_\noisetime}{\latent_\noisetime}$, $\mathcal{A}_\phi$ is the parameterized forward model, $\sigma$ is the standard deviation of the additive observation noise, $\decodeNote^*$ is the pre-trained latent decoder, and $\mathbb{E}[{\latent}_{0}| \latent_{t}]$ can be estimated through a reverse time SDE from $\latent_{t}$~\cite{chung2022diffusion}.
%However, simply adopting Eq.~\ref{equ: blindinverse1} does not work, as the latent space to pixel space is not a one$\to$one mapping. 
% In fact, such LDMs for posterior sampling are notorious for the artifacts due to the vulnerability of latent space~\cite{rout2024solving, chung2023prompt}
Due to the fact that latent space to pixel space is not a one-to-one mapping, the data likelihood term could pull $\boldsymbol{z}_{t}$ to many potential $\boldsymbol{z}_{0}$ in different directions. To alleviate this risk, we introduce an additional "gluing" regularization to enhance training stability as suggested by~\cite{rout2024solving}:
\begin{equation}
\begin{aligned}
 	\scoreFunc{\latent_\noisetime}{\latent_\noisetime \mid \observation}
    &  \approx \pretrainSdModel{(\latent_\noisetime, \noisetime)} - \frac{1}{2\sigma^{2}} \nabla_{\mathbf{x}_{t}}\left\|\mathbf{y}-\mathcal{A}_\phi\left( \pretraiedDecodeFunc{\mathbb{E}[{\latent}_{0}| \latent_{t}]}\right)\right\|_{2}^{2} \\
    & + \gamma\nabla_{z_{t}}\left\|\mathbb{E}\left[\boldsymbol{z}_{0}|\boldsymbol{z}_{t}\right]-\mathcal{E}^*\left(\mathcal{A}_\phi^{T} \mathcal{A}_\phi \hat{\boldsymbol{x}}_{0}+\left(\boldsymbol{I}-\mathcal{A}_\phi^{T} \mathcal{A}_\phi\right) \hat{\boldsymbol{x}}_{0}\right)\right\|^{2},
\label{equ: guling}
\end{aligned}
\end{equation}
where $\encodeNote^*$ is the pre-trained latent encoder, $\gamma$ weights the "gluing" regularization, and $\hat{\boldsymbol{x}}_{0}=\mathcal{D}^*(\mathbb{E}\left[\boldsymbol{z}_{0}| \boldsymbol{z}_{t}\right])$.
However, Eq.~\eqref{equ: guling} works only when $\forwardFunc_\forwardParam$ is known, \ie, non-blind settings~\cite{rout2024solving}.  In the context of blind inversion, $\forwardFunc_\forwardParam$ is randomly initialized so that significant modeling errors perturb the optimization of $\boldsymbol{z}_t$ in the latent space. Consequently, there are significant artifacts when directly applying Eq.~\ref{equ: guling}. %, as shown in Fig.~\ref{fig:exp-aba-annealing}(b). 
%
We have to introduce an annealing technique to stabilize the training process:
% suppress the optimization artifacts.
%
\begin{technique}  [Annealed consistency.]
	Suppose that the estimated forward operator $\mathcal{A}_\phi$ is optimized from coarse to fine in the iterations, we have that:
    \begin{equation}
		\resizebox{1.0\hsize}{!}{$	\scoreFunc{\latent_\noisetime}{\latent_\noisetime \mid \observation}
    \approx \pretrainSdModel{(\latent_\noisetime, \noisetime)} - \frac{1}{2\zeta_t \sigma^2} \nabla_{\mathbf{x}_{t}}\left\|\mathbf{y}-\mathcal{A}_\phi\left( \pretraiedDecodeFunc{\mathbb{E}[{\latent}_{0}| \latent_{t}]}\right)\right\|_{2}^{2} + \gamma\nabla_{z_{t}}\left\|\mathbb{E}\left[\boldsymbol{z}_{0}|\boldsymbol{z}_{t}\right]-\mathcal{E}^*\left(\mathcal{A}_\phi^{T} \mathcal{A}_\phi \hat{\boldsymbol{x}}_{0}+\left(\boldsymbol{I}-\mathcal{A}_\phi^{T} \mathcal{A}_\phi\right) \hat{\boldsymbol{x}}_{0}\right)\right\|^{2},$}
			\label{equ: scale-up}
	\end{equation}
 
	% \begin{equation}
	% 	\resizebox{1.0\hsize}{!}{$	\scoreFunc{\latent_\noisetime}{ \observation \mid \latent_t} \approx
	% 		\frac{1}{\zeta} \left[ 	\scoreFunc{\latent_\noisetime}{ \observation \mid \pretraiedDecodeFunc{\mathbb{E}[{\latent}_{0}| \latent_{t}]} } 
	% 		+ \gamma\nabla_{z_{t}}\left\|\mathbb{E}\left[\boldsymbol{z}_{0}|\boldsymbol{z}_{t}\right]-\mathcal{E}^*\left(\mathcal{A}_\phi^{T} \mathcal{A}_\phi \hat{\boldsymbol{x}}_{0}+\left(\boldsymbol{I}-\mathcal{A}_\phi^{T} \mathcal{A}_\phi\right) \mathcal{D}^*\left(\mathbb{E}\left[\boldsymbol{z}_{0}| \boldsymbol{z}_{t}\right]\right)\right)\right\|^{2} \right] ,$}
	% 		\label{equ: scale-up}
	% \end{equation}
	where $\zeta_t$ is a time-dependent factor that scales up over time, \eg, it anneals linearly from 10 at $t=1000$ to 1 at $t=400$ and then holds
	\label{technique:annealing}
\end{technique}
We refer to this scaling technique as \textit{annealed consistency}. Intuitively, $\forwardFunc_\forwardParam$ is randomly initialized at the beginning, which cannot provide correct gradient directions. Therefore, we reduce its influence on the evolution of $\boldsymbol{z}t$ with a large factor ($\zeta=10$). As training progresses, $\forwardFunc_\forwardParam$ gradually aligns with the underlying true forward operator. We then anneal the factor ($\zeta=1$) to enforce data consistency. We find that this annealing technique is critical for blind inversion with latent priors; without it, the optimized signal $\signal$ consistently exhibits severe artifacts, as shown in Figure~\ref{fig:exp-aba-annealing}. Further theoretical explanations can be found in Appendix~\ref{app:anneal}.

\vspace*{-0.2cm}
\subsection{M-step: Forward Operator Estimation}
\label{sec:M-step}
The goal of  {\name}’s M-step is to update the forward operator parameters $\forwardParam$ with the estimated samples $\hat{\signal}_0$ from the E-step. %, that is, estimate the forward operator $\mathcal{A}_{\phi}$.
This can be achieved by solving a maximum-a-posterior (MAP) estimation problem:
\vspace*{-0.1cm}
\begin{equation}
    \forwardParam^* = \arg \max _{\phi}\left[ \log p_\forwardParam(\observation \mid \hat{\signal}_0) +\log \probDistribution{\forwardParam}\right] = \arg \min_{\phi} \left[|| \observation-\forwardFunc_\forwardParam(\hat{\signal}_0) ||^2_2  + \mathcal{R}(\phi)\right], 
\label{Equ: map}
\end{equation}
where $\probDistribution{\forwardParam}$ is the prior distribution of $\phi$, and $\mathcal{R}(\forwardParam)$ is an equivalent regularizer. $\mathcal{R}(\forwardParam)$ can include sparsity, patch-based priors, plug-and-play denoisers~\cite{pan2016l_0, sun2013edge}, etc. This MAP estimation problem can be solved using either gradient-based optimization~\cite{laroche2024fast} or neural networks~\cite{chung2022parallel}. Compared to BlindDPS~\cite{chung2022parallel}, which jointly optimizes 
$\signal$ and $\forwardParam$ using two diffusion processes, our method leverages the properties of EM~\cite{gao2021deepgem}, resulting in faster convergence and better performance.

%Typically, Monte Carlo sampling can be applied to draw $N$ samples in the E-step and aggregrate their infomation to solve the best forward operator parameters $\forwardParam^* $.  In practice, we find one sample is enough, thanks to the powerful diffusion process. 
%
% For general blind inverse problems, 
% Our EM framework provides a general framework to update $\forwardParam$ iteratively, depending on the corresponding blind inverse tasks. It supports $\probDistribution{ \observation | \hat{\signal}_0, \forwardParam }$ to be either updated by an implicit neural network approximation~\cite{chung2022parallel} or traditional optimization schemes~\cite{laroche2024fast}. 
%We show $\forwardParam$. different blind inverse tasks and derive different algorithms to update 
% Compared to BlindDPS~\cite{chung2022parallel} which jointly optimize $\signal$ and $\forwardParam$ using two diffusion processes, our method inherits properties of EM~\cite{gao2021deepgem} which is faster and yields better convergence. 


\vspace*{-0.2cm}
\subsection{Scheduling of E-steps and M-steps}
\label{sec:EM framework}

We propose a scheduling strategy for the E-steps and M-steps tailored to latent blind inversion tasks to significantly accelerate the optimization process. The E-step comprises three sub-steps: prior-based diffusion, data likelihood-based diffusion, and gluing regularization, where the first happens in latent space while the rest happen in pixel space that requires encoder-decoder operations. Our key observation is that LatentDEM's time consumption is primarily due to the encoder-decoder functions (\ie, $\signal  = \mathcal{D}^*(\latent)$ and $\latent = \mathcal{E}^*(\signal)$) , particularly their gradient computations. This occurs in the data likelihood and gluing terms in the E-step and the data likelihood term in the M-step.

In the early stages of the diffusion process, the sampled data is far from the true value, making frequent LDM encoding and decoding unnecessary. Instead, $\latent_t$, can rely on LDM priors to diffuse for several steps. Therefore, we can safely skip gradient computations to accelerate the process to diffuse for several steps. Therefore, we can safely skip gradient computations to accelerate the process, 

% especially their gradient computation. This occurs in the data likelihood term and gluing term in the E-step and the data likelihood term in the M-step. However, in the early stages of the diffusion process, the sampled data is far from the true value, making it unnecessary to compute LDM encoding and decoding processes frequently in the early stage, as such information is not accurate. Instead, $\latent_t$ can rely only on the LDM priors ($\scoreFunc{\latent_t}{\latent_z}$) to diffuse for several steps. Therefore, we can safely skip the gradient computation for accelerating, which we called skip gradient technique.

% which occur in both the E-step and the M-step. In the early stages of the diffusion process, the sampled data is far from the true value, making it unnecessary to update the model parameters (run the M-step) after each E-step. Instead, we can safely skip some M-step computations, particularly the gradient computations for model parameter estimation, thereby accelerating the process. which contains the annealed consistency term(Eq.~\ref{equ: scale-up}) in the E-step, as well as the whole M-step. Specifically, these terms mainly contributes to $\scoreFunc{\latent_t}{\observation | \latent_t}$ and $\forwardParam$.
%
% However, in the beginning of the optimization, the sampled data is far from the true value. 
% Besides the annealing technique, 
%and have applied the annealing teachnique(Tech.~\ref{technique:annealing}) to reduce the influence of the noisy gradients. 
% Therefore, we argue that it is not necessary to compute LDM encoding and decoding processes frequently in the early stage, as such information is not accurate. Instead, $\latent_t$ can rely more on the LDM priors only($\scoreFunc{\latent_t}{\latent_z}$). Therefore, we can safely skip the computation burden and propose a skip gradient technique for accelerating.
% 最优值
\begin{technique}  [\text{Skip Gradient}]
	In early stages ($t>\skipEnd$), %, where $\skipEnd=800$),
	 performing  $\skipNum$ times half E-step in latent space with $	\scoreFunc{\latent_\noisetime}{\latent_\noisetime}$ only, then perform the whole EM-step in both latent space and image space. We typically set $\skipEnd=200$ and $\skipNum=10$, which means we skip $M=(T-\skipEnd)(1-1/\skipNum)=(1000-200)(1-1/10)=720$ full gradient computation steps .
\end{technique}

\vspace*{-0.1cm}
We refer to this new technique as \textit{skip gradient}.  Intuitively, at early stages, due to the fact that both sampled data $\hat{\signal}_0$ and the forward parameters are not accurate, it is unnecessary to enforce data consistency and update forward operators at each reverse timestep.
%
We show such a skip technique significantly reduces computation overhead while keeping PSNR values approximate to the non-skip version, as demonstrated in Figure~\ref{fig:exp-aba-skip}. Our algorithm is describe in Algorithm~\ref{algo:1}.

%That is, the generative process of LDMs is decoupled with the estimation of forward operators, accelerating the EM iterations by skipping certain encoder-decoder computation and gradient computation.
%Since LatentDEM essentially performs joint optimization via LDMs and an EM algorithm (up to the variational approximation), our method inherits properties of EM~\cite{gao2021deepgem}, including convergence to a local minimum of Eq.~\ref{Equ: map}.



% TODO 哪一步是E-step，哪一步是M-step
% 1. E-step factor, M-step general, accelerating
% 一行列两个算法（blinddps latentdem
% \begin{algorithm}
% 	\begin{algorithmic}[1]
% 		\caption{LatentDEM for Blind Inverse Problems}
% 		\label{algo:1}
% 		\REQUIRE $T, \boldsymbol{y}, \{\eta_i\}_{i=1}^T, \{\gamma_i\}_{i=1}^T, \{\tilde{\sigma}_i\}_{i=1}^T, \mathcal{E}, \mathcal{D}, A\tilde{x}_0, A, \boldsymbol{s}_\theta$
% 		\STATE $\boldsymbol{z}_T \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{I})$
% 		\FOR{$i = T - 1$ \textbf{to} $0$}
% 		\STATE $ \boldsymbol{s} \leftarrow \boldsymbol{s}_0(\boldsymbol{z}_i, i)$
% 		\STATE $\tilde{\boldsymbol{z}}_0 \leftarrow \frac{1}{\sqrt{\tilde{\alpha}_i}} (\boldsymbol{z}_i + (1 - \tilde{\alpha}_i)\boldsymbol{s})$
% 		\STATE $\epsilon \sim \mathcal{N}(0, I)$
% 		\STATE $\boldsymbol{z}'_{i-1} \leftarrow \frac{\sqrt{\alpha_i}(1-\tilde{\alpha}_{i-1})}{1-\tilde{\alpha}_i} \boldsymbol{z}_i + \frac{\sqrt{\tilde{\alpha}_{i-1}\beta_i}}{1-\tilde{\alpha}_i} \tilde{\boldsymbol{z}}_0 + \tilde{\sigma}_i \epsilon$
% 		\STATE $\Tilde{x}_0 = D(\tilde{\boldsymbol{z}}_0)$
% 		\STATE $A_{i-1} = Mstep(\boldsymbol{y},\tilde{x}_0,\lambda,\beta, \sigma)$ 
% 		\textcolor{blue}{\COMMENT{Details in Sec.~\ref{sec:M-step}}}
% 		\STATE $\boldsymbol{z}''_{i-1} \leftarrow \boldsymbol{z}'_{i-1} - \eta_i \nabla_{\boldsymbol{z}_i} \lVert \boldsymbol{y} - A(D(\tilde{\boldsymbol{z}}_0)) \rVert^2$
% 		\STATE $\boldsymbol{z}_{i-1} \leftarrow \boldsymbol{z}''_{i-1} - \gamma_i \nabla_{\boldsymbol{z}_i} \lVert \tilde{\boldsymbol{z}}_0 - E(A^T A \tilde{x}_0 + (I - A^T A)\mathcal{D}(\tilde{\boldsymbol{z}}_0)) \rVert^2$
% 		\ENDFOR
% 		% \STATE \textbf{return} $D(\tilde{z}_0)$
		
% 	\end{algorithmic}
% \end{algorithm}

% Common choices for $p(\phi)$ are sparsity priors $l0$~\cite{pan2016l_0},$l1$, $l2$ and patch-based priors~\cite{sun2013edge}. Though these priors are simple and efficient, they do not fit the scenarios where measurement noise rises~\cite{laroche2024fast}. In this paper, we adopt a plug-and-play denoiser to serve as the prior. 

% Take blind deblurring for example, we train a simple DnCNN~\cite{zhang2017beyond} on kernels generated by~\cite{gavant2011physiological}.

% For general blind inverse problems, the solution of the measurement consistency term $p(\boldsymbol{y}| \phi, \hat{\boldsymbol{x}_0}^{(i)})$ can be approximated by a deep neural network implicitly. 

\subsection{Blinding Inversion Tasks}
\label{sec:app}
% here is the separate 2 algorithms
% only one，突出改的地方，不能太长

\input{Styles/chapter/fig-2-alg}

Our framework incorporate powerful LDM priors within the EM framework, which enables solving both linear and non-linear inverse problems.  We showcase two representative tasks: the 2D blind debluring task, and the  high-dimension, non-linear 3D blind inverse rendering problem. 

%
\textbf{2D Blind Deblurring} \ \ \ 
In the blind deblurring task, our goal is to jointly estimate the clean image and the blur kernel given a blurry observation. In E-step the image is sampled in LDMs. In M-step, we adopt Half-Quadratic Splitting (HQS) optimization scheme~\cite{geman1995nonlinear, laroche2024fast} to estimate kernels explicitly.
Blur kernel estimation has been a well-studied deconvolution procecess where HQS solves it in the Fourier domain followed by a neural denoiser~\cite{zhang2017beyond}:
\begin{equation}
\resizebox{0.8\hsize}{!}{$
    \mathbf{Z}^{(t-1)}=\textit{F}^{-1}(\frac{\textit{F}(\observation)\textit{F}(\hat{\signal}_0^{(t)})+\beta\sigma^2\textit{F}(\forwardParam^{(t)})}{\textit{F}^{2}(\hat{\signal}_0^{(t)})+\beta\sigma^2}), \ \ \ \ \ 
	\forwardParam^{(t-1)} =\mathbf{D}_{\sqrt{\lambda/\beta}}(\mathbf{Z}^{(t-1)}),
 $}
	\label{eq:hqs2}
\end{equation}
where $\sigma$ denotes the noise level of measurements, $\lambda$ and $\beta$ are constant hyperparameters to help HQS converge~\cite{zhang2021plug} , $\textit{F}$ and $\textit{F}^{-1}$ denote Fourier transform and inverse fourier transform, $\mathbf{Z}$ is a intermediate variable and $\mathbf{D}$ is a plug-in-play neural denoiser~\cite{laroche2024fast}, respectively. We use the superscript $^{(t-1)}$ and $^{(t)}$ to denote the iteration update.% Eq.~\ref{eq:hqs1} and Eq.~\ref{eq:hqs2} are performed iteratively in a single M-step till convergence.

\textbf{Pose-free Sparse-view 3D Reconstruction} \ \ \ 
%
%
For the first time, we show blind inversion can also be applied in the challenging sparse-view, unposed 3D reconstruction  task.
%
We utilize Zero123~\cite{liu2023zero1to3}, which fine-tune stable diffusion model with multi-view images and implicitly learns the underlying 3D knowledge, \eg, it supports generating multi-view images that describe the 3D object information. 
%
Zero123 can be formulated as $\hat{\image} = \forwardFunc_\cameraParam(\image)$, where given an input image $\image$ and its relative camera rotation and translation parameters $\cameraParam=(R, T)$,  it produces the corresponding novel-view image $\hat{\image}$.  However, Zero123 operates in a feed-forward model and starts from a single image to generate all the rest views, which suffers from  accumulated view inconsistency errors.

%
We reformulate Zero123 as pose-free, sparse-view blind 3D inversion task, where the novel view images and the camera parameters are jointly optimized from sparse-view input images. We tackle a two-view reconstruction setting but more views yield better performance. Given two  images $\image_1$ and $\image_2$ without knowing their poses, we first apply Zero123 to create a novel view image $\hat{\image}$ from $\image_1$, where $\hat{\image} = \forwardFunc_{\cameraParam_1}(\image_1)$ and $\cameraParam_1$ is a user-defined target view. At the same time, we also optimize another  camera parameter $\hat{\cameraParam}_2$, such that the generated image $\hat{\image}$ can also be produced by $\image_2$ with  $\hat{\cameraParam}_2$: % $\image^{\cameraParam_1}= \forwardFunc_{\cameraParam_2}(\image_2)$.  We apply below method
\begin{comment}
    \hat{\image}^* &= \arg \max _{\hat{\image}} \probDistribution{\hat{\image} | \image_1, \cameraParam_1, \image_2, \hat{\cameraParam}_2} 
	 \label{equ: pose image_estimation} 
	 \\
\end{comment}
\begin{equation}
    \hat{\image}^* = \arg \max _{\hat{\image}} \probDistribution{\hat{\image} | \forwardFunc_{\cameraParam_1}(\image_1) , \forwardFunc_{ \hat{\cameraParam}_2}(\image_2)}, \ \ \ \ 
    \hat{\cameraParam}_2^{(t-1)} \approx \hat{\cameraParam}_2^{(t)} -
	\nabla_{\cameraParam_2^{(t)}}|| \boldsymbol{y}-\mathcal{A}_{\hat{\cameraParam}_2^{(t-1)}}\hat{\boldsymbol{x}_0}^{(t-1)} ||^2_2
	\label{equ: pose estimation}
\end{equation}

Note that in the E-step(Eq.~\eqref{equ:image_estimation}), we do not run two diffusion steps but aggregate information from both $\image_1$ and $\image_2$ to produce a more consistent image $\image_{\cameraParam_1}$~\cite{bibid}. In the M-step(Eq.~\eqref{equ:estimation}),  $\cameraParam_2$ is optimized via a gradient disecnt manner. The brings two advantages: first, our method frees the pose requirement in 3D reconstruction. Second, by aggregating multi-view information in the E-step, we produce much more consistent novel view images. We show our results not only outperform the state-of-the-art pose-free sparse-view 3D baselines~\cite{leap}, but also generate well-aligned images that can be used to create delicate 3D models~\cite{representations}. More details are provided in Supp.

